Hybrid Alignment Training for Large Language Models

Alignment training is crucial for enabling large language models (LLMs) to cater to human intentions and preferences. It is typically performed based on two stages with different objectives: instruction-following alignment and human-preference alignment. However, aligning LLMs with these objectives in sequence suffers from an inherent problem: the objectives may conflict, and the LLMs cannot guarantee to simultaneously align with the instructions and human preferences well. To response to these, in this work, we propose a Hybrid Alignment Training (Hbat) approach, based on alternating alignment and modified elastic weight consolidation methods. The basic idea is to alternate between different objectives during alignment training, so that better collaboration can be achieved between the two alignment tasks.We experiment with Hbat on summarization and dialogue tasks. Experimental results show that the proposed \textsc{Hbat} can significantly outperform all baselines. Notably, Hbat yields consistent performance gains over the traditional two-stage alignment training when using both proximal policy optimization and direct preference optimization.

==> figures/radar_analysis.tex <==
\makeatletter
\def\tkz@KiviatGrad[#1](#2){% 
\begingroup
\pgfkeys{/kiviatgrad/.cd,
graduation distance= 0 pt,
prefix ={},
suffix={},
unity=1,
% added the following four lines
label precision/.store in=\gradlabel@precision,
label precision=1,
zero point/.store in=\tkz@grad@zero,
zero point=0
}
\pgfqkeys{/kiviatgrad}{#1}% 
\let\tikz@label@distance@tmp\tikz@label@distance
\global\let\tikz@label@distance\tkz@kiv@grad
  % started loop at zero, to get label for center point
  \foreach \nv in {0,...,\tkz@kiv@lattice}{
  % skipped the \pgfmathparse, moved
  % \tkz@kiv@unity*\nv-\tkz@grad@zero
  % into \pgfmathsetmacro. The last term is added
  \pgfmathsetmacro{\result}{\tkz@kiv@unity*\nv+20} % change from \pgfmathtruncatemacro
  % NOTE: use \gradlabel@precision for the precision
  \protected@edef\tkz@kiv@gd{%
    \tkz@kiv@prefix%
    \pgfmathprintnumber[precision=\gradlabel@precision,fixed]{\result}%% used \pgfmathprintnumber instead of "$\result$"
    \tkz@kiv@suffix} 
    \path[/kiviatgrad/.cd,#1] (0:0)--(360/\tkz@kiv@radial*#2:\nv*\tkz@kiv@gap)
      % NOTE: (360/\tkz@kiv@radial*#2)-90  -> (360/\tkz@kiv@radial*#2)
      % removed 90 because you rotate all the diagrams
      node[label=(360/\tkz@kiv@radial*#2):\tiny\tkz@kiv@gd] {}; % added \tiny
  }
  \let\tikz@label@distance\tikz@label@distance@tmp  
\endgroup
}%


\def\tkz@KiviatLine[#1](#2,#3){% 
\begingroup
\pgfkeys{/kiviatline/.cd,
fill= {},
opacity=.5,
% add these two lines, similar to for kiviatline
zero point/.store in=\tkz@line@zero,
zero point=0
}
%
% the code below has a lot of polar coordinates, of the form
%   (angle: <value> * <some factor>)
% all have been modified to get them on the form
%   (angle:{(<value>+\tkz@line@zero) * <some factor>})
% note extra braces, which are required when a component contains ()
% 
\pgfqkeys{/kiviatline}{#1}%   opacity ??????
\ifx\tkzutil@empty\tkz@kivl@fill \else 
\begin{scope}[on background layer]
  \path[fill=\tkz@kivl@fill,opacity=\tkz@kivl@opacity] (360/\tkz@kiv@radial*0:{(#2+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step})   
  \foreach \v [count=\rang from 1] in {#3}{%  
   -- (360/\tkz@kiv@radial*\rang:{(\v+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step}) } -- (360/\tkz@kiv@radial*0:{(#2+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step}); 
\end{scope}
\fi       
% added overlay option because something weird happened with the bounding box
\draw[#1,opacity=1,overlay] (0:{(#2+\tkz@line@zero)*\tkz@kiv@gap}) plot coordinates {(360/\tkz@kiv@radial*0:{(#2+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step})}  
\foreach \v [count=\rang from 1] in {#3}{%  
 -- (360/\tkz@kiv@radial*\rang:{(\v+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step}) plot coordinates {(360/\tkz@kiv@radial*\rang:{(\v+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step})}} -- (360/\tkz@kiv@radial*0:{(#2+\tkz@line@zero)*\tkz@kiv@gap*\tkz@kiv@step});   
\endgroup
}%  

\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{c1}{HTML}{81BECE}
\definecolor{c2}{HTML}{378BA4}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{global scale/.style={
    scale=#1,
    every node/.append style={scale=#1}
  }
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[
  label distance=13em,
  global scale = 0.73,
  plot1/.style={
    thin,
    draw=c1,
    fill=c1,
    mark=square*,
    mark options={
     ball color=blue, % note ball color inside mark options
     mark size=4pt
    },
    opacity=.5
  },
  plot2/.style={
    thin,
    draw=c2,
    fill=c2,
    mark=triangle*,
    mark options={
      mark size=4pt,
      ball color=blue
    },
    opacity=.5
  },
  plot3/.style={
    thin,
    draw=red!30,
    fill=red!30,
    mark=square*,
    mark options={
      mark size=4pt,
      ball color=yellow
    },
    opacity=.5
  },
  plot4/.style={
    thin,
    draw=red!50,
    fill=red!50,
    mark=triangle*,
    mark options={
      mark size=4pt,
      ball color=blue
    },
    opacity=.5
  }
]
%%%%%%%%%%%%%%%%设置画布大小%%%%%%%%%%%%%%%%%%%%%%%%
\useasboundingbox (-25em,-5em) rectangle (10em,7em);
% Correlation coefficient
\begin{scope}[scale=0.36,local bounding box=a,shift={(-50em,0)}]

% define some macros for convenience
\newcommand\KivStep{0.1}
\pgfmathsetmacro\Unity{1/\KivStep}
\newcommand\zeroshift{20.00}

 \tkzKiviatDiagram[
   radial  style/.style ={-},
   rotate=90, 
   lattice style/.style ={black!30},
   step=\KivStep,
   gap=1,
   lattice=5,
]% 
% de$\rightarrow$en  en$\rightarrow$de
{cs$\rightarrow$en,cs$\rightarrow$it,,ro$\rightarrow$en,en$\rightarrow$cs,it$\rightarrow$cs,,en$\rightarrow$ro,cs$\rightarrow$en}
\node [align=center,rotate=90]at (0em,16em){de$\rightarrow$en};
\node [align=center,rotate=270]at (0em,-16em){en$\rightarrow$de};

% with tm
\tkzKiviatLine[
  % /kiviatline/zero point=\zeroshift,
  plot3
](38.58,27.93,39.74,39.66,32.58,27.22,33.56,30.18)
% wo tm
\tkzKiviatLine[
  % /kiviatline/zero point=\zeroshift,
  plot4
](17.50,7.02,21.37,16.34,8.02,2.85,7.06,8.74)

\tkzKiviatGrad[unity=\Unity, label precision=2, zero point=\zeroshift](0) % set unity as 0.1
\end{scope}
%PBIAS
\begin{scope}[scale=0.36,local bounding box=b,shift={(-15em,0)}]

\newcommand\KivStep{0.1}
\pgfmathsetmacro\Unity{1/\KivStep}
\newcommand\zeroshift{20.00}

 \tkzKiviatDiagram[
   radial  style/.style ={-},
   rotate=90,
   lattice style/.style ={black!30},
   step=\KivStep,
   gap=1,
   lattice=5
]% 
% it$\rightarrow$en en$\rightarrow$it
{es$\rightarrow$en,fr$\rightarrow$en,,de$\rightarrow$fr,en$\rightarrow$es,en$\rightarrow$fr,,fr$\rightarrow$de}
\node [align=center,rotate=90]at (0em,16.5em){it$\rightarrow$en};
\node [align=center,rotate=270]at (0em,-16.5em){en$\rightarrow$it};
% with tm
\tkzKiviatLine[
  % /kiviatline/zero point=\zeroshift,
plot1
](41.25,44.45,41.80,33.52,39.18,44.60,37.71,30.08)
% wo tm
\tkzKiviatLine[
  % /kiviatline/zero point=\zeroshift,
plot2
](21.89,24.06,21.13,14.78,17.10,23.78,13.53,8.93)
%%%%%%%%
\tkzKiviatGrad[unity=\Unity, zero point=\zeroshift](0) % set unity as 0.1
\end{scope}

\end{tikzpicture}



==> tables/vicuna-80.tex <==
\begin{tabular}{lccc}
    \toprule[1.1pt]
    Category \ \ \ & SFT & DPO \\ \midrule
    Generic         &8.28    &8.22 ($+$0.06)                \\
    Knowledge       &8.00    &9.20 ($+$1.20)                \\ 
    Roleplay        &8.17	 &7.71 ($-$0.46)		        \\ 
    Common-sense    &8.29	 &8.68 ($+$0.39)		        \\ 
    Fermi           &3.13	 &2.78 ($-$0.35)		        \\
    Counterfactual \ \ \ \ \ \ \ \ &5.57	 &5.23 ($-$0.34)    \\
    Coding          &3.00	 &4.00 ($+$1.00)		        \\
    Math            &2.50	 &1.33 ($-$1.17)	             \\
    Writing         &6.67  	 &8.33 ($+$1.66)	               \\
    \bottomrule[1.1pt]
\end{tabular}

% ['generic', 'knowledge', 'roleplay', 'common-sense', 'fermi', 'counterfactual', 'coding', 'math', 'writing']
